Improving Entity Resolution with Global Constraints

Some of the greatest advances in web search have come from leveraging socio-economic properties of online user behavior. Past advances include PageRank, anchor text, hubs-authorities, and TF-IDF. In this paper, we investigate another socio-economic property that, to our knowledge, has not yet been exploited: sites that create lists of entities, such as IMDB and Netflix, have an incentive to avoid gratuitous duplicates. We leverage this property to resolve entities across the different web sites, and find that we can obtain substantial improvements in resolution accuracy. This improvement in accuracy also translates into robustness, which often reduces the amount of training data that must be labeled for comparing entities across many sites. Furthermore, the technique provides robustness when resolving sites that have some duplicates, even without first removing these duplicates. We present algorithms with very strong precision and recall, and show that max weight matching, while appearing to be a natural choice turns out to have poor performance in some situations. The presented techniques are now being used in the back-end entity resolution system at a major Internet search engine.

==> subfiles/2-Problem.tex <==
\section{One-to-One Resolution} \label{sec:problem}
 
We begin with a description of the abstract entity resolution problem, before specializing to globally constrained resolution. Let \DB{1} and \DB{2} be two \term{datasets} each containing a finite number of \term{rows} representing \term{entities}. The dataset sizes need not be the same, and each dataset represents its entities via an encoding in some set $\Domain_i$. The goal of the \term{Entity Resolution Problem} is to identify an unknown target relation or \term{resolution} $\TargetMatch \subseteq \DB{1} \times \DB{2}$, given some information about \TargetMatch. In practice a retrieved relation $\PredictedMatch\subseteq\DB{1}\times\DB{2}$ is deemed to be a good approximation of \TargetMatch\ if it has high precision and recall.

In the common supervised scenario for entity resolution, a subset of resolutions $\TargetMatch_{train,+}\subset\TargetMatch$ and possibly also a subset of non-resolutions $\TargetMatch_{train,-}\subset \left(\DB{1}\times\DB{2}\right)\backslash \TargetMatch$ are known and the goal of entity resolution reduces to learning $\PredictedMatch \approx \TargetMatch$ given these example pairs. Most commonly this is accomplished as a supervised regression or classification problem by learning a scoring function $f:\Domain_1 \times\Domain_2 \to \Reals$ such that \PredictedMatch\ is taken to be all pairs in $\DB{1}\times\DB{2}$ with a score above a given threshold $\theta\in\Reals$. In the absence of a labeled training set, expert knowledge about the datasets and their domains may yield a similar scoring function.

We focus on the important case of \term{one-to-one entity resolution}. In the exact one-to-one case, the target \term{matching} \TargetMatch\ is one-to-one: for each $x_1\in\DB{1}$ there exists at most one $y\in\DB{2}$ such that $(x_1,y)\in\TargetMatch$, and similarly for each $y_2\in\DB{2}$ there exists at most one $x\in\DB{1}$ such that $(x,y_2)\in\TargetMatch$. 

The added structure of the one-to-one resolution problem suggests that the task be viewed in terms of graph matching as follows. The edge set $\DB{1}\times\DB{2}$, together with the vertices $\DB{1}\cup\DB{2}$ form a complete bipartite graph. Target \TargetMatch\ now corresponds to a subset of edges that forms a matching in the graph theoretic sense. Clearly, a resolution \PredictedMatch\ that attempts to approximate \TargetMatch\ should be constrained to be one-to-one, which is in stark contrast with existing approaches in the entity resolution literature. Maximum cardinality matching, for example, involves finding a generic resolution that optimizes a global objective function. One-to-one constrained resolution sets the seemingly more difficult goal of finding a specific resolution (that is possibly far from maximum in cardinality). 

As in the general entity resolution problem, one-to-one resolution begins with learning a scoring function $f$, which represents similarity between entities in each dataset, or the likelihood of a match. Given these scores, the complete bipartite graph becomes weighted; and assuming scores that \emph{well approximate} the likelihood of a match, retrieving \TargetMatch\ can be seen as selecting edges of high weight. However unlike the general entity resolution problem, the selection of high weight edges should be globally constrained to be one-to-one. Moreover just as one-to-one entity resolution differs to maximum cardinality, the problem is related but different to maximum weight graph matching: since $|\TargetMatch|$ may be far less than the sizes of either dataset, it is in general undesirable to match all rows from either \DB{1} or \DB{2}. Given an appropriate score function, \emph{low-scoring edges, even if they satisfy the global one-to-one constraint without blocking high-scoring edges, should not be included in the matching \PredictedMatch}.

Many of the ideas of this section translate naturally into simple yet effective algorithms for the one-to-one resolution problem.
